SkyCell: A Space-Pruning Based Parallel Skyline Algorithm

Skyline computation is an essential database operation that has many applications in multi-criteria decision making scenarios such as recommender systems. Existing algorithms have focused on checking point domination, which lack efficiency over large datasets. We propose a grid-based structure that enables grid cell domination checks. We show that only a small constant number of cells need to be checked which is independent from the number of data points. Our structure also enables parallel processing. We thus obtain a highly efficient parallel skyline algorithm named SkyCell, taking advantage of the parallelization power of graphics processing units. Experimental results confirm the effectiveness and efficiency of SkyCell -- it outperforms state-of-the-art algorithms consistently and by up to over two orders of magnitude in the computation time.

==> fig/pgfbegin.tex <==
\usepackage{times,amsmath,epsfig}
\usepackage{latexsym}
\usepackage{graphicx}
\pagestyle{empty}

\usepackage{amssymb}
\usepackage{graphicx}

\def\xcolorversion{2.00}
\def\xkeyvalversion{1.8}
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,snakes,calc,automata,backgrounds,petri,matrix,patterns,shapes.arrows,positioning,through}
\usetikzlibrary{intersections}

\begin{document}

\begin{tikzpicture}[scale=.4, thick, help lines/.style={thin,
    draw=black!50}, line join=round, >=stealth']
 

==> fig/pgfend.tex <==

\end{tikzpicture}
\end{document}


==> fig/wallstyle.tex <==
\tikzset{ voronoi/.style={fill=black!40},tdash/.style={dashed, white!60!black,
    very thick}, tsolid/.style={black,opacity=.5, very
    thick},tred/.style={red,opacity=.5, very
    thick},onn/.style={tdash},tnn/.style={tsolid}, bnn/.style={tsolid}}
